Disentangled Acoustic Fields For Multimodal Physical Scene Understanding

We study the problem of multimodal physical scene understanding, where an embodied agent needs to find fallen objects by inferring object properties, direction, and distance of an impact sound source. Previous works adopt feed-forward neural networks to directly regress the variables from sound, leading to poor generalization and domain adaptation issues. In this paper, we illustrate that learning a disentangled model of acoustic formation, referred to as disentangled acoustic field (DAF), to capture the sound generation and propagation process, enables the embodied agent to construct a spatial uncertainty map over where the objects may have fallen. We demonstrate that our analysis-by-synthesis framework can jointly infer sound properties by explicitly decomposing and factorizing the latent space of the disentangled model. We further show that the spatial uncertainty map can significantly improve the success rate for the localization of fallen objects by proposing multiple plausible exploration locations.

==> figtext/teaser.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.45\linewidth]{iclr2024AuthorKit/fig/teaser2.pdf}
\caption{\textbf{Audio inference in humans.} Upon hearing a glass bottle fall to the ground, we humans can instinctively infer information about its material, direction, and distance, and react accordingly. The goal of this work is to construct an analysis-by-synthesis loop, and enable similar capabilities for embodied agents.}
\label{teaser}
\vspace{-1.2em}
\end{figure}

==> sections/01_Intro.tex <==
\section{Introduction}
% Jonathan, thanks for taking a look at the paper. I've made a pass over the methods section and unified the notation per your suggestions.
% yilundu: I would maybe use this intro format:
% yilundu: First talk about how audio perception is very important, for instance for navigation. Talk about how neural acoustic fields enables us to accurately capture audio
% yilundu: Next paragraph: Neural acoustic fields enables us to synthesize different possible audio sounds at different location. But another major question is how we may use it for perception -- for instance how we can infer where objects
% yilundu: fall.
% yilundu: Third paragraph: we propose a method based off a loss surface of rendering, then talk about how it enables multimodal navigation




Imagine walking through a forest with your eyes closed, listening to the sounds around you. As you move, you hear the rustling of leaves as an animal passes by, the gentle bubbling of a nearby stream, and the soft whisper of the wind. These sounds provide valuable information about the environment. Sound waves are influenced by the objects they encounter, changing in timbre, direction, and intensity as they reflect, diffract, and absorb. As humans, we intuitively understand how sound behaves in physical spaces, enabling us to infer the presence, location, and physical properties of objects from the sounds we hear. 
% By incorporating audio information into multimodal scene understanding, we can gain deeper insights into the physical world and develop more robust models for applications such as robotics, autonomous vehicles, and virtual and augmented reality.




% Close your eyes, and listen closely as you walk in a forest. You may hear the crackling of leaves as an animal moves, the bubbling of a small river, and the whisper of the wind. As sound travels through an environment and encounters obstacles and structures, it is occluded and reflected, it may gain reverberation or have its timbre changed. You may not see any of these objects, but you can intuitively reason about what objects were responsible for a sound, its direction, and how far it has travelled. But beyond straightforward judgements, humans have the ability to reason about the underlying physical mechanisms that produce what is heard. Standing next to a sound-reflective surface, we know that sounds that we hear are likely reflected and not emitted from the surface. Not only can we make use of uncertainty, we can also incorporate this information into our understanding of the physical world.

Recent progress in neural fields has yielded high-fidelity models of perceptual modalities such as vision, touch, and sound. Most recently, neural acoustic fields (NAFs)~\cite{luo2022learning} propose representing spatial acoustics of sounds, enabling continuous modeling of sound propagation and reverberation in a given scene. By modeling such acoustics, NAFs implicitly capture the structure and material properties of a scene. However, NAFs are overfitted to the acoustic properties of a single room, preventing them from being used as a disentangled model of sound across many environments.


% \begin{figure}[htbp]
% 		\centering
% 		\includegraphics[width=0.8\linewidth]{iccv2023AuthorKit/fig/teaser2.pdf}
% 		\caption{Upon hearing a glass bottle fall to the ground, a person can instinctively infer its material, direction and distance, and react accordingly.}
% 		\label{teaser}
% 	\end{figure}




% \input{iclr2024AuthorKit/figtext/teaser}


In this work, we propose disentangled acoustic fields (DAFs), an approach to modeling acoustic properties across a multitude of different scenes. In NAFs, the short-time Fourier transform (STFT) of audio reverberation is the object of the modeling, but it is highly sensitive to the geometry of each scene and thus difficult to fit across different scenes. Instead, DAFs seek to model object sounds across multiple scenes using the power spectral density (PSD). This approach provides a lower dimensional compact representation of acoustics that preserves much of the physical information in emitted sounds. We demonstrate the effectiveness of this approach by showing high-accuracy object property inference across a set of different scenes.


We demonstrate how DAFs can be used to effectively enhance audio perception. Specifically, we propose using DAFs as a ``mental simulation engine'' that can test different physical scene configurations to identify the world state that best matches the given sound. This ``analysis-by-synthesis'' approach allows us to robustly infer the underlying locations of fallen objects and effectively navigate to locate them. Our experiments show that, by using DAFs, we can accurately identify categories of fallen objects and their locations, even in complex acoustic environments.

Acoustic rendering with DAFs further enables us to obtain an uncertainty measure of different physical scene parameters, such as object locations, by assessing the mismatch between a simulated sound and ground-truth sound. We illustrate how such uncertainty may be used in the task of finding a fallen object, where we may naturally generate plans to different goals by considering the underlying uncertainty cost. In summary, our contributions are as follows:
\vspace{-1mm}
\begin{itemize}[align=right,itemindent=0em,labelsep=2pt,labelwidth=1em,leftmargin=*,itemsep=0em] 
	\item We introduce Disentangled Acoustic Fields (DAFs), an approach to model acoustic properties across a multitude of different scenes.
	\item  We illustrate how analysis-by-synthesis using DAFs enables us to infer the physical properties of a scene.
	\item We illustrate how we may use DAFs to represent uncertainty and to navigate and find fallen objects.
\end{itemize}




% While NAFs can render spatial audio with high fidelity, the model is designed to capture the sound propagation in a single scene and does not explicitly facilitate acoustic reasoning. In order to utilize an implicit neural field for the localization of fallen objects, we seek to simultaneously address two long-standing problems. First, an embodied agent needs to perform reasoning across multiple novel scenes and orientations, without any a priori knowledge of the scene it is currently located in. Two, we seek to explicitly model the uncertainty of the emitter location. While it may be tempting to invert NAFs, the underdetermined character of the system means that it is impossible to solve for the original raw sound and emitter location given a recording.

% While in theory NAFs may be ``inverted'' given a sound captured at the listener, due to the underdetermined character of the system, it is impossible to uniquely solve for the original raw sound and emitter location. 

% To accurately model . In contrast to NAFs, we model the power spectral density (PSD) of acoustic propogation, a lower dimensional subspace of acoustics which may more accurately represent
% To address both challenges, we propose a system that explicitly leverages a generative acoustic field as a model used for acoustic reasoning across multiple scenes, and can directly represent the uncertainty map of plausible locations for a given object. As our system utilizes egocentric coordinates, we amortize the inference of scene properties into the network training itself. Our formulation uses the signal at the listener as input, jointly decomposes the signal into components like category, material, location, and latent, and represents the appropriateness of a location using a reconstruction loss in spectral density. By doing so, the network learns to model the uncertainty present in the acoustic information. The modular nature of our design lends itself to %modular
% combinations with complementary methods. We illustrate the efficacy of our in localizing fallen objects given only emitted sound.






% Listen closely as an object falls under the influence gravity. It makes a characteristic 

% Modern AI technologies have achieved considerable success in pattern recognition tasks, yet they still fall short when it comes to tasks involving physical reasoning and interaction. This is mainly due to a lack of innate, human-like, multi-sensory modeling. In reality, humans combine multi-sensory information to perceive and interact with the environment. For instance, humans respond to a knock by walking to the door and opening it. Unfortunately, current AI systems are not able to function as general-purpose reasoning modules in such complex tasks. To address this issue and promote progress, a variety of novel embodied AI tasks have been proposed. Among them, we are interested in the audio-visual navigation, which is a complex and challenging embodied AI task.
%  Unlike visual navigation \cite{wijmans2019dd}, an audio sound source is used to define the target, and the agent must use both audio and visual signals to navigate to the target \cite{chen2021semantic,gan2020look, chen2020learning}. Recently a challenging task \cite{gan2022finding} is introduced for an agent to find fallen object in a room. Some state-of-the-art navigation systems perform poorly in this challenge, including SAVi \cite{chen2021semantic}, Decision TransFormer \cite{chen2021decision} and Object-Goal \cite{chaplot2020object}.
% In his paper, \cite{gan2022finding} has implemented a hybrid and modular baseline framework that integrates the auditory perception module and the visual semantic mapping module. 
% The modular planning approach outperforms other methods but still fails to find the object in the given steps in many cases. A key bottleneck is accurately predicting object categories from audio alone, which suggests that the trained auditory perception module failed to learn to effectively infer the physics from sound. On the other hand, if the agent fails to find the object near the predicted position, it adopts a frontier exploration strategy to search in unexplored areas, resulting in a significant number of extra steps being required before arriving at the right object position.



% To solve aforementioned issues, we propose an uncertainty-based method to improve the search efficiency in the aid of the neural acoustic field. To this end, we train a variant auto-encoder (VAE) to learn an object-centric neural implicit function as a generative model to approximate an object’s sound based on its physical properties. Specifically, the encoder receives the short time Fourier transform spectrogram encoded from the impulse response of auditory input and predicts the object type, material, position, and spatial latents which represent local geometric information, near either emitter or listener locations. The decoder then receives the object material, position, spatial latent, and reconstructs the power spectral density of the auditory input. We further generate an uncertainty map based on the reconstruction loss of the neural acoustic field, and adapt the A-star algorithm to our framework for path planning. Our main contributions are summarized as follows:




==> sections/02_Related.tex <==
\section{Related Work}

\subsection{Neural Implicit Representations}
Learned implicit functions have emerged as a promising representation of the 3D geometry~\cite{luo2021surfgen, park2019deepsdf,qu2024implicit}, appearance~\cite{mildenhall2021nerf,sitzmann2019scene}, and acoustics of a scene~\cite{luo2022learning}. Unlike traditional discrete representations, implicit functions compactly encode information in the weights of a neural network, and can continuously map from spatial coordinates to output. Recent work has proposed to encode shapes as signed distance fields, learn appearance with differentiable rendering, and render acoustics by generating spectrograms \cite{xie2022neural} \cite{luo2022learning}. For acoustics, \cite{du2021learning} proposed to jointly generate acoustics and images by sampling from a joint manifold, and \cite{luo2022learning} introduced the concept of Neural Acoustic Fields (NAFs), an implicit representation that captures sound propagation in a physical scene. While NAFs enable the modeling of sounds at novel locations in a single scene, they cannot be generalized to enable reasoning across novel scenes. In contrast, our method can generalize to novel scenes at test time, enables joint inference of object properties and location, and allows uncertainty-aware object localization. 

% Recently, neural implicit representation has become a focus in computer vision research, and high-quality representations of the visual world \cite{sitzmann2019scene,wang2021nerf} have been developed. These models typically employ a neural renderer and a learned implicit representation to jointly capture and render images of a scene. Multi-view consistency between visual observations is leveraged in order to infer images of the same scene from novel viewpoints. Additionally, progress has been made in learning spatial auditory representations. For example, \cite{luo2022learning} introduces Neural Acoustic Fields (NAFs), an implicit representation that captures sound propagation in a physical scene. Experiments show that the continuous nature of NAFs allows us to render spatial acoustics for a listener at any location, and that it can accurately predict sound propagation at novel locations. In this work, we learn an object-centric neural implicit function as a generative model to approximate an object's sound based on its physical properties.



\subsection{Multimodal Scene Understanding}

Recent work has explored the use of input modalities beyond vision alone for scene understanding\cite{yin2021m2dgr,yin2024ground}. Extensive studies have demonstrated the effectiveness of integrating audio and visual information in diverse scene understanding applications \cite{zhang2018inverting,owens2016ambient, owens2018learning, zhu2021deep}. For instance, \cite{ephrat2018looking,zhao2018sound,gao2018learning} employ visual input to separate and localize sounds, \cite{gao2020visualechoes} leverages spatial cues contained in echoes for more accurate depth estimation, while \cite{chen2021structure,luo2022learning,arandjelovic2017look, owens2018audio} demonstrate the potential of sound in learning multimodal features and inferring scene structure. Cross-modal generation has gained increasing attention by researchers~\cite{gan2020foley, owens2016visually, su2020audeo, chen2017deep}. Furthermore, \cite{afouras2020self,gan2019self, arandjelovic2018objects} integrate both visual and auditory information to localize target objects more accurately. Motivated by these findings, we propose a disentangled acoustic field for physical scene understanding, where an embodied agent seeks to find fallen objects by inferring their physical properties, direction, and distance from an impact sound.


\subsection{Audio-Visual Navigation}

Our work is also closely related to audio-visual navigation, where navigation is achieved using audio signals to augment vision \cite{chen2021semantic,chen2019audio,gan2020look}. In particular, \cite{chen2020soundspaces} proposed the AudioGoal challenge, where an embodied agent is required to navigate to a target emitting a constant sound using audio for positional cues \cite{chen2020learning}. Building on this, \cite{chen2021semantic} introduced the novel task of semantic audio-visual navigation, in which the agent must navigate to an object with semantic vision and short bursts of sound. However, their dataset had one limitation: it did not include synthesis capability for impact sound and thus could not render the physical properties (like material, position) by audio. To address both issues, \cite{gan2022finding} proposed the Find Fallen Object task, where physical reasoning was combined with sound. This dataset was based on the TDW~\cite{gan2020threedworld} simulation platform, which can generate audio from a variety of materials and parameters, and utilizes Resonance Audio \cite{resonanceaudio} (a technology for accurately replicating how sound interacts with the environment in 3D spaces) to spatialize the impact sounds depending on the room's spatial dimensions and wall/floor materials. Considering these advantages, we choose it as the benchmark to assess the capability of our proposed method on multi-modal physical scene understanding. 

% Audio was rendered with TDW’s PyImpact Python library, which uses modal synthesis to generate audio from information about the material types and impact parameters of colliding objects (velocities, normal vectors, and masses). Impact sounds were then spatialized using Resonance Audio, providing reverberation simulation that reflects the spatial dimensions of the room and the wall and floor materials being used. Considering these advantages, we choose this dataset to evaluate our proposed method.

% have been used to plan actions directly from raw sensory
% data perform poorly. In our work, we aim to build an agent can accurately predict the object type and position while achieving the goal efficiently.




% Motivated by these findings, we investigate a generative acoustic field for physical scene understanding, where an embodied agent seeks to find fallen objects by inferring their properties, direction, and distance from an impact sound source.




% \subsection{Target-driven Navigation}
% Towards visual navigation, researchers have developed algorithms that use egocentric vision to travel to a designated point in a new environment \cite{wijmans2019dd,gupta2017cognitive,chaplot2020learning} or search for a specified object \cite{chaplot2020neural,savinov2018semi,zhu2017visual}. To expand the sensory suite of the navigating agent, Chen et al. \cite{chen2020soundspaces} proposed the AudioGoal challenge, which requires an agent to navigate to a constantly sounding target (e.g. an alarm chirping) using audio for key directional and distance cues \cite{chen2020learning}. Building on this, \cite{chen2021semantic} introduced a novel task: semantic audio-visual navigation, wherein the agent must navigate to an object situated contextually in an environment that only makes sound for a certain period of time. However, this dataset had two limitations: first, it did not include impact sound synthesis capability and thus was unable to render the physical properties and interactions of objects via audio, and second, the sounding source locations were defined in 2D uniform grids with fixed height, rather than the 3D locations that characterize sound source localization in real-world environments. To address these limitations, \cite{gan2022finding} proposed Find Fallen Object, a new embodied AI challenge for multi-modal physical scene understanding. As described before, deep learning–based methods
% have been used to plan actions directly from raw sensory
% data perform poorly. In our work, we aim to build an agent can accurately predict the object type and position while achieving the goal efficiently.










 


% \section{Methodology}

% \subsection{Variational Autoencoder}
% % In our work, we learn an object-centric neural implicit function as a generative model to approximate an object’s sound based on its physical properties, and to adopt an analysis-by-synthesis approach to invert the object physics from sound.

% Variational autoencoder (VAE) \cite{kingma2013auto} is a widely used generative model developed from the standard autoencoder. It typically encodes the input data $x$ into a latent space $z$ with Gaussian distributions, and then samples data points from the latent space to construct the input data via a decoder. 
% The goal of VAEs is to train a network in the form of $p(\boldsymbol{x}, \boldsymbol{z})=p(\boldsymbol{z}) p(\boldsymbol{x} \mid \boldsymbol{z})$ where $p(\boldsymbol{z})$ is a prior distribution over latent variables $\boldsymbol{z}$ and $p(\boldsymbol{x} \mid \boldsymbol{z})$ is the likelihood function or decoder that generates data $\boldsymbol{x}$ given latent variables $\boldsymbol{z}$. Since the true posterior $p(\boldsymbol{z} \mid \boldsymbol{x})$ is in general intractable, the generative model is trained with the aid of an approximate posterior distribution or encoder $q(z \mid x)$.



% Due to the nature of generative models, variational autoencoders can be used for semi-supervised learning, which was first proposed in [15] (named Semi-VAE). In this model, both the input data $x$ and its label $y$ are used for learning the latent variable $z$ via an encoder $q_\phi(z \mid x, y)$, where $\phi$ denotes its parameters. The decoder then constructs input data using a distribution $p_\theta(x \mid y, z)$, where $\theta$ is the decoder parameters. The task label predictor distribution is denoted as $q_\phi(y \mid x)$. The distribution of the latent variable $z$ is derived as follows:

==> sections/03_Methods.tex <==


\section{Proposed Method}
\input{figtext/generative_model}
We are interested in learning a disentangled framework of sound that can effectively generalize across scenes, object types, and object locations. Key to our approach is an explicitly decomposed latent space that models the individual contribution of the sound factors. We first describe the parameterization of our disentangled acoustic field, which simultaneously enables factorization of the sound generation process and is defined on continuous locations in space. We further characterize the design choices that enable robust generalization and describe how we can use the continuous nature of our disentangled acoustic field to facilitate the localization of a fallen object.

\subsection{Physics of Sound}
\label{secformation}
Given the sound of a falling object received by an agent as binaural signal $s$, we seek to identify the relative egocentric object location $p \in \mathbb{R}^{3}$, the object material category $m \in \{1, 2, \dots, M\}$, the object type category $t \in \{1, 2, \dots, T\}$, and a low-dimensional latent code $z \in \mathcal{R}^{k}$, where $z$ can contain information that is independent from the previous factors, such as information about the scene structure, scene materials, and properties about the propagation medium. Given an accurate model of sound formation $G$, we seek to reconstruct the sound via $G(p, m, t, z)$. In practice, we here do not reconstruct the sound itself, but its power spectral density, a simplified representation encompassing essential properties about the falling object.

% In our approach, we denote the input feature of spectrogram as $\mathbf{x_s}$. The physical audio information including objcet type, material and position
% is denoted as $z$. The goal of the neural implicit representation model is to learn an neural acoustic representation $\mathbf{r}_f$ for each sample from $\mathbf{x_s}$, where its physical information $\mathbf{z}$ can be minimally inferred from its representation $\mathbf{r}_f$. In addition, the representations should be maximally informative for predicting the physical audio information. 




% \begin{table}
% \label{variable}
% \caption{The main variable denotations in our method.}
% \centering
% \begin{tabular}{cl}
% \hline Variable & \multicolumn{1}{c}{ Description } \\
% \hline $\mathbf{x_s}$ & Input spectrogram \\
% $\mathbf{x_p}$ & Input power spectral density \\
% $\hat{\mathbf{x}}_p$ & Reconstructed power spectral density \\
% $\mathbf{t}$ & Real object type \\
% $\hat{\mathbf{t}}$ & Predicted object type \\
% $\mathbf{m}$ & Real object material \\
% $\hat{\mathbf{m}}$ & Predicted object material \\
% $\mathbf{p}$ & Real object position related to agent\\
% $\hat{\mathbf{p}}$ & Predicted object position related to agent\\

% $\mu$ & Mean vector of latent space \\
% $\sigma$ & Co-variance vector of latent space \\
% $\mathbf{h}$ & Latent Representation \\
% $\mathbf{c}$ & Combined hidden representation \\
% $\mathcal{L}_T$ & Object type prediction loss \\
% $\mathcal{L}_M$ & Object material loss \\
% $\mathcal{L}_P$ & Object position loss \\
% $\mathcal{L}_{KLD}$ & Kullback-Leibler divergence (KLD) loss \\
% $\mathcal{L}_R$ & Reconstruction loss \\
% \hline
% \end{tabular}
% \end{table}


\subsection{Disentangled Acoustic Fields (DAFs)}



We aim to learn a disentangled model of sound formation that facilitates efficient inference for characterizing sound properties. The parameterization of sound formation introduced in Section~\ref{secformation} provides a general framework for building such a disentangled model. To enhance effective learning, we structure our framework using an encoder, denoted as $E_{\omega}$, and a generator, denoted as $G_{\phi}$. By instructing the network to consider the relative egocentric location of the sound emitter, we guide it to disregard the absolute positions of the agent and object, and reason in a generalizable fashion.


Given a sound signal represented as a binaural waveform $s \in \mathbb{R}^{2\times t}$, we process the signal using the short-time Fourier transform (STFT), and retain the log-magnitude as $S$. Following prior work, we discard the phase present in the original signal, which is difficult to model~\cite{du2021learning,luo2022learning}. We further investigated the choice of output representation, and found that the STFT of a fallen object sound used in prior work~\cite{gan2022finding} includes large irregular stretches of uninformative silence along the time domain. The irregular and unpredictable temporal gaps are difficult for a neural network to effectively estimate and reconstruct, and in practice, a full-fidelity reconstruction of the sound signal in the original domain may not be necessary, as our ultimate goal is the inference of the underlying factors of sound formation.  We thus transform the sound from the waveform domain into power spectral density (PSD) representation $\bar{S}$ using Welch's method  (basically an average pooling over time of the squared STFT magnitude) as a target for our generator, which retains crucial information on the power present in each frequency, but collapses the information along the time dimension.

We may thus model the latent factors as the outputs of an encoder $E_{\omega}$ which takes as input the sound representation $S$:
\begin{align}
    (\hat{p}, \hat{m}, \hat{t}, \hat{\mu}, \hat{\sigma}) = E_{\omega}(S); \quad \hat{z} \sim \mathcal{N}(\hat{\mu}, \hat{\sigma}^2\cdot\mathbb{I}),
\end{align}
where we model $\hat{z}$ as a sample from a diagonal Gaussian with mean $\hat{\mu}$ and standard deviation $\hat{\sigma}$. This restricted parameterization prevents the encoder from compressing all sound information into $\hat{z}$. The generator $G_{\phi}$ is modeled as a neural field which takes as input the latent factors and attempts to generate the PSD:
\begin{align}
    \hat{\bar{S}} = G_{\phi}(\hat{p}, \hat{m}, \hat{t}, \hat{z}).
\end{align}
We train our network with supervision on the latent factors and the output. For the $i$-th training example, we have access to the ground truth location, object material, and object type as the tuple $(p_i, m_i, t_i)$.

\input{figtext/entire_model}
The object type and material are supervised with cross-entropy loss:
\begin{align}
    \mathcal{L}_\text{type}&=\text{CrossEntropy}(\mathrm{t}_i,\hat{\mathrm{t}}_i),\\
    \mathcal{L}_\text{material}&=\text{CrossEntropy}(\mathrm{m}_i,\hat{\mathrm{m}}_i),
\end{align}
where $\mathrm{t}_i$  and  $\mathrm{m}_i$  are the ground-truth object type and material for the $i$-th training sample, and $\hat{\mathrm{t}}_i$ and $\hat{\mathrm{m}}_i$ their estimates. 
% We will later utilize the position vector in the inference of our loss surface. 
An MSE loss is applied to facilitate the learning of the position vector:
\begin{align}
\mathcal{L}_\text{position}=\frac{1}{2} \sum_i\left\|\hat{{p}}_i-{p}_i\right\|_2^2.
\end{align}
During training, we sample from the posterior for a given sound $S_{i}$ modeled as a multivariate Gaussian with diagonal covariance:
\begin{align}
    q_{\omega}(z|S_{i}) := \mathcal{N}(z; \mu_{i}, \sigma^2_i\cdot\mathbb{I})
\end{align}
We apply the reparameterization trick~\cite{kingma2013auto} to allow for backpropagation through the parameters $\mu_{i}, \sigma_{i}$, by setting $z_i = \mu_i + \sigma_i \odot \epsilon$, where $\epsilon \sim \mathcal{N}(0, \mathbb{I})$. The latent $z$ is regularized with:
\begin{align}
    D_\text{KL}(q_{\omega}(z|S_i)||\mathcal{N}(0, \mathbb{I}))
\end{align}
The output of the generator is supervised with an MSE loss to facilitate the prediction of the PSD:
\begin{equation}
\mathcal{L}_\text{PSD}=\frac{1}{d} \sum_i\left\|\hat{\bar{S}}_i-\bar{S}_i\right\|^2,
\end{equation}
where $d$ is the dimension of the output PSD feature. 
In summary, our overall objective is to minimize:
\begin{equation}
    \mathcal{L}_\text{total} = \alpha \mathcal{L}_\text{type} + \beta \mathcal{L}_\text{material} + \gamma \mathcal{L}_\text{position} 
    +  \delta D_\text{KL} + \eta  \mathcal{L}_\text{PSD},
\end{equation}
where $(\alpha, \beta, \gamma, \delta, \eta)$ are hyperparameters.




% We attempt to map the audio data space to a new space containing physical audio information such as object type and location. To achieve this, we adopt an auto-encoder network, which provides a non-linear mapping function that is learned iteratively through encoder and decoder components. Directly outputting the impulse-response with a neural network is difficult due to its chaotic nature and high dimensionality. To avoid this problem, we instead encode the impulse-response utilizing a short-time Fourier transform (STFT) to create a log-magnitude spectrogram, which is found to be significantly more amenable to neural network prediction \cite{luo2022learning}, due to its smoother nature in the frequency space. 

% \paragraph{Network Architecture}
% We adopt ResNet-50~\cite{he2016deep} as our encoder backbone. The input layer is modified to accept two channel images corresponding to the left/right spectrograms in the binaural input. We take the output of the global pooling layer as output, and learn linear projection layers to output the position of the object $q$, the categorical variable $asd$, as well as $\mu$ and $\sigma$ which we use to parameterize a normal distribution with diagonal covaraince.

% The generator is composed of a stack of fully connected layers. The network accepts as input the concatenated latent factors 

% We adapt ResNet-50 \cite{he2016deep} as the backbone of our encoder network, which consists of six stages. The first stage consists of a 7x7 convolutional layer, followed by a batch normalization layer and a LeakyReLU \cite{maas2013rectifier} activation layer. This is followed by four stages of convolutional layers, each composed of a series of bottleneck blocks with three convolutional layers, including a 1x1 convolutional layer to reduce the number of channels in the input, a 3x3 convolutional layer, and a 1x1 convolutional layer to increase the number of channels. These layers act as a "bottleneck" to reduce the parameters and improve training speed. The output of each block is then passed through a shortcut connection, allowing the gradient to pass through the network more quickly, resulting in improved performance. The last stage is a global average pooling layer that outputs a single vector and a fully-connected layer to predict the different physical information and latent space features.
% By contrast, the decoder model is composed of a number of fully connected layers, beginning with an input layer of size 20, followed by three residual layers, and ending with an output layer of size 258. The residual layers, each composed of two linear layers and two LeakyReLU layers, help the model learn more complex features by allowing it to approximate more complex functions. The LeakyReLU layers introduce a small amount of non-linearity into the model to help it capture more complex patterns. The output layer is used to generate the reconstructed PSD from the model.



% During training, we sample a latent code $z$ from the approximate posterior for a given shape $x_j$ modeled as a multivariate Gaussian with diagonal covariance:
% \begin{equation}
% q\left(z \mid x_j\right):=\mathcal{N}\left(z ; \mu_j, \sigma_j^2 \cdot \mathbb{I}\right)
% \end{equation}


% We use the reparameterization trick [26] to allow for direct optimization of latent parameters $\mu_j, \sigma_j$, and set $z_j=$ $\mu_j+\sigma_j \odot \epsilon$, where $\epsilon \sim \mathcal{N}(0, \mathbb{I})$. During training, the generator and latent parameters are trained to minimize the the adversarial objective $\mathcal{L}_{G A N}$ and maximize the evidence lower bound of the marginal likelihood (ELBO):
% $$
% \begin{aligned}
% \log p_\theta(x) & \geq \underset{z \sim q(z \mid x)}{\mathbb{E}}[\log p(x \mid z)]-D_{K L}(q(z \mid x) \| p(z)) \\
% p(x \mid z) & \left.=-\underset{\mathbf{p}}{\mathbb{E}}\left[\mathcal{L}_{S D F}\left(g_\psi(z, \mathbf{p}), \operatorname{SDF}_s(\mathbf{p})\right)\right)\right]
% \end{aligned}
% $$





% The object type loss and material loss are formulated as follows, respectively:
% % \begin{equation}
% % \mathcal{L}_T=-\sum_i \mathrm{t}_i \log \left(\hat{\mathrm{t}}_i\right)
% % \end{equation}

% \begin{equation}
% \mathcal{L}_T=CrossEntropy(\mathrm{t}_i,\hat{\mathrm{t}}_i)
% \end{equation}
% % \begin{equation}
% % \mathcal{L}_M=-\sum_i \mathrm{m}_i \log \left(\hat{\mathrm{m}}_i\right)
% % \end{equation}
% \begin{equation}
% \mathcal{L}_M=CrossEntropy(\mathrm{m}_i,\hat{\mathrm{m}}_i)
% \end{equation}
% where $\mathrm{t}_i$ / $\mathrm{m}_i$ and $\hat{\mathrm{t}}_i$ / $\hat{\mathrm{m}}_i$ are the true and predicted object type / material for the $i$-th class. 

% We apply an MSE loss of the predicted position and the ground-truth position to the encoder to optimize its ability in inferring object position, which is denoted as follows:

% \begin{equation}
% \mathcal{L}_P=\frac{1}{d} \sum_i^d\left(\hat{\mathbf{p}}_i-\mathbf{p}_i\right)^2,
% \end{equation}
% where where $\mathrm{p}_i$ and $\hat{\mathrm{p}}_i$ represent the true and predicted object position for the $i$-th class, respectively. And the KLD loss is calculated by:

% \begin{equation}
% \mathcal{L}_{KLD}=-\frac{1}{2} \sum_i^n(1+\sigma-\mu^2-\exp{\sigma}),
% \end{equation}
% where $\mu$ and $\sigma$ denote mean vector and co-variance of latent space, which are computed by:
% \begin{equation}
% \mu=f(\mathbf{U} \mathbf{x}+\mathbf{u})
% \end{equation}

% \begin{equation}
% \sigma=f(\mathbf{W} \mathbf{x}+\mathbf{w})
% \end{equation}
% where $\mathbf{W}, \mathbf{w}, \mathbf{U}$ and $\mathbf{u}$ are parameters, $f(\cdot)$ is the activation function. The latent representation $h$ is sampled from the latent space spanned by $\mu$ and $\sigma$ via reparameterization as follows:
% \begin{equation}
% \mathbf{h}=\mathcal{N}(0, \mathbf{I}) * \sigma+\mu
% \end{equation}


% The latent representation is further concatenated with the  predicted physical audio information to form a union $\mathbf{c}=[\tilde{\mathbf{t}}, \hat{\mathbf{m}},\hat{\mathbf{p}}, \mathbf{h}]$. It is used to reconstruct the PSD through a decoder model. To train the decoder model to make accurate PSD reconstruction, we apply a reconstruction $\operatorname{loss}^1$ to the reconstructed feature $\hat{\mathbf{x}}_p$, which is denoted as follows:
% \begin{equation}
% \mathcal{L}_R=\frac{1}{d} \sum_i^d\left(\hat{\mathbf{x}}_i-\mathbf{x}_i\right)^2,
% \end{equation}
% where $d$ is the dimension of input PSD feature. 
% We train our model on the Find Fallen dataset \cite{gan2022finding} using the joint loss:
% \begin{equation}
% \mathcal{L}_{total}=\mathcal{L}_{T} + \mathcal{L}_{M}+\mathcal{L}_{P}+\mathcal{L}_{R}+\mathcal{L}_{KLD},
% \end{equation}



\subsection{Inference of Sound Parameters}
We seek to invert the model of sound generation and compute the factors responsible for a given sound. Our disentangled model enables us to use ``analysis by synthesis'' to render all different acoustics parameters and find the one which matches our sound the best. However, the combinatorial complexity of enumerating combinations of factors renders this process computationally prohibitive. Instead, we amortize the inference of type, material, and latent into the joint learning process of the encoder and generator. We focus our efforts on the inference of object position, which is composed of continuous variables and is critical for the localization of the fallen object.


\vspace{2mm}
\noindent\textbf{Loss Map Generation:}
Given a sound $s$ as recorded by an embodied agent, we use the encoder to infer the material, type, and continuous latent. We define a search space $10$~m $\times$ $10$~m centered on the agent position, and discretize this space using a resolution of $0.1$~m. Using the previously inferred type, material, and Gaussian latent, we iterate over all possible locations $p_j$ where the object could be located. The current iterated position is combined with the other factors as inferred by the encoder network and provided to the generator. The pipeline is shown in Algorithm~\ref{algo}.
% \begin{algorithm}[h]
% \caption{Inferring a loss map of positions}
% \textbf{Input:} Sound as log-mag.~STFT $S$ and PSD $\bar{S}$\\
% \hspace{10.1mm} Encoder network $E_{\omega}$, generator network $G_{\phi}$\\
% \hspace{10.1mm} Loss map grid $\mathcal{L}_\text{grid}$\\
% \hspace{10.1mm} Function $f_{r2g,c, \theta}$ for global coordinates
% \\
% 1: $(\hat{{p}}, \hat{{m}},\hat{{t}}, {\hat{z}}) = E_{\omega}(S)$\\
% 2: for $x_\text{pos}$ in $[-5\text{ m}, +5\text{ m}]$:\\
% 3: \hspace{4.5mm}for $y_\text{pos}$ in $[-5\text{ m}, +5\text{ m}]$:\\
% 4:\hspace{9mm} $\hat{{p}} = (x_\text{pos}, y_\text{pos})$\\
% 5:\hspace{9mm}$\mathcal{L}_\text{grid}[f_{r2g,c, \theta}(\hat{{p}})]= (G_{\phi}([\hat{{p}}, \hat{{m}},\hat{{t}}, {\hat{z}}])-\bar{S})^2$
% \end{algorithm}
% \newline\noindent 

The generated PSD is compared against the ground-truth PSD $\bar{S}$ of the sound of the fallen object, and an MSE difference is recorded at each location. In this fashion, we may generate a loss map corresponding to the two-dimensional coordinates. Since the loss map is based on the egocentric neural acoustic field, we need to convert the relative coordinates to the global frame of the room for path planning:
% In each falling object experiment, we first predict its type, material and location based on the audio signal. Then we traverse a 10m*10m space with a resolution of 0.1m, combine each coordinate with the previously predicted information and input it into the decoder network to reconstruct the power spectral density of the audio. Finally, we calculat the MSE loss between reconstructed PSD and real PSD. In this way, we get a loss surface corresponding to the two-dimensional coordinates. Since the uncertainty map is based on the egocentric neural acoustic field, We need to convert the relative coordinates to the global frame of the room where the agent is located:

\begin{equation}
\resizebox{0.87\columnwidth}{!}{$
f_{r2g, c,\theta}\left(\left[\begin{array}{l}
x \\
y
\end{array}\right]\right)
=\left[\begin{array}{l}
x^{\prime} \\
y^{\prime}
\end{array}\right]=\left[\begin{array}{cc}
\cos \theta & -\sin \theta \\
\sin \theta & \phantom{-}\cos \theta
\end{array}\right]\left[\begin{array}{l}
x \\
y
\end{array}\right]+\left[\begin{array}{l}
c_x \\
c_y
\end{array}\right]$}
\end{equation}
 where $(c_x,c_y)$ is the agent's current position in the global frame and $\theta$ is its rotation angle in the global frame, while $(x,y)$ is the coordinate in the agent's egocentric frame.

\vspace{2mm}


\noindent\textbf{Uncertainty-Aware Planning:}
We adopt a modular approach to path planning~\cite{gan2022finding}. Given the audio, we predict the object type and location via $E_{\omega}$. We further construct an internal model of the world from RGB-D images of the environment. Semantic segmentation is computed using a pre-trained Mask-RCNN~\cite{he2017mask} model as illustrated in Figure~\ref{simulation}. We use the depth map to project the semantic map into world space. Given the object types as inferred by the encoder network, we take the top-$3$ object type candidates (local minimas) as search targets. 
If a target is visible to the agent when initialized, the agent attempts to navigate to the location of the visible object. If there is no target in view, the agent will navigate to the predicted position. If the first attempt fails, the agent updates the world model and searches for potential object candidates. Object candidates are ranked according to the loss map value at the location corresponding to each object. Once the target list is determined, we apply the $A^*$ algorithm \cite{hart1968formal} to plan the shortest collision-free path to the first target in an unvisited area of the map.

% For the initial attempt, the agent will navigate to location of the target object if it is directly in view; otherwise navigate to the predicted position by the encoder network.
% If the first attempt fails, the agent updates the world model and ranks 
% potential object candidates according to the loss map value at the location corresponding to each object. Once the target list is determined, we apply the $A^*$ algorithm \cite{hart1968formal} to plan the shortest collision-free path to the first target in an unvisited area of the map.


\input{tabletext/algo}

% Firstly, the model predicts the fallen object’s losscategory and location based on the audio. Secondly, it builds maps of the environment from RGBD images in search of the fallen object. We adopt the Mask-RCNN model \cite{he2017mask} as a visual perception module for
% semantic segmentation of 30 object types. We put the three most likely objects on the shortlist. 
% If no corresponding object type in view, the agent movies towards the point with minimum loss on the uncertainty map to find potential objects. If finding multiple objects with the predicted type, we find the closest point on the loss surface to the central coordinate point of the connection domain of these objects, the robot then determines a target list from lowest to highest based on the loss value of the nearest point. Once the target list is determined, we apply the A-Star algorithm \cite{hart1968formal} to plan a shortest path to the first target in a collision-free and unvisited area of the map.




% 1. Predicting the object location and type from audio information. Also generating an uncertainty map based on reconstruction loss.
% 2. If no corresponding object type in view, moving close to the point with minimum loss on the uncertainty map.
% 3.If finding multiple objects with the predicted type, traversing these points based on their loss value
% 4.Once the goal is determined, A-star algorithm is adopted to search a closest path to the goal


==> sections/04_Results.tex <==




\section{Experiment}

\subsection{Inference of Object Properties}


To test the physical inference capability of our proposed model, we first evaluate it on the Find Fallen Dataset \cite{gan2022finding} and compare it against two baselines. The first is the modular sound predictor presented in \cite{gan2022finding}, which was learned without the use of a disentangled model. 
The second is a gradient-based optimization process that minimizes the difference between the predicted and ground-truth PSD by optimizing all latent factors using our trained generator. All methods are evaluated on the same test split. To enable exploring multiple plausible locations, we mark a type as accurately predicted if the correct object type is within the top-$3$ predicted categories. The results in Table~\ref{accuracy} show that our model significantly outperforms the baseline methods in both position and type prediction accuracy. By jointly learning a disentangled model along the encoder, we can more accurately predict the object location and the object type. Gradient-based optimization fails in jointly optimizing the position and object type, and is easily stuck in local minima.

% \subsection{Evaluation on OBJECTFOLDER2 Dataset}
% \label{sect:objectfolder}

We evaluate our model on the OBJECTFOLDER2 \cite{gao2022objectfolder} dataset, which contains 1000 virtualized objects with different sizes and types along with acoustic, visual, and tactile sensory information. Correspondingly, we adjust the output of the encoder network and the input of the decoder network to correspond to the object scale and type. As indicated in Table~\ref{objectfolder}, our method surpasses the performance of the baseline approach \cite{gao2022objectfolder}, which employs a ResNet-18 architecture utilizing the magnitude spectrogram as input to predict the object scale and type.

\input{tabletext/objectfolder}


We further extend our evaluation to the REALIMPACT dataset \cite{clarke2023realimpact}, encompassing 150,000 impact sound recordings across 50 $\textbf{real-world}$ object categories. This dataset incorporates impact sounds captured from 600 distinct listener locations, spanning 10 angles, 15 heights, and 4 distances. We use the same train/test split across all methods. To accommodate with the dataset, we adapt the output of the encoder network and the input of the generator network to be angle, height, and distance. The official baseline method is a ResNet-18 network employing the magnitude spectrogram of impact sounds to predict the corresponding object properties.  As highlighted in Table~\ref{realimpact}, our method demonstrates a significant improvement over baseline methods in predicting the category of object angle, height, and distance.

\input{tabletext/accuracy_compare}
\input{tabletext/realimpact}
\input{figtext/topdown}


% \vspace{2mm}
% \noindent\textbf{Navigation and Planning.}


\subsection{Navigation and Planning}
\noindent\textbf{Experimental Setup.}
We use the TDW \cite{gan2020threedworld} simulation platform to evaluate our proposed method. Our networks are trained on the Find Fallen Object dataset\footnote{https://github.com/chuangg/find$\_$fallen$\_$objects}, following the experimental configuration described in \cite{gan2022finding}. This dataset contains 8000 instances of 30 physical object types in 64 physically different rooms (32 study rooms and 32 kitchens). We evaluated the models' performance on the test split identified by \cite{gan2022finding}. The audio was only available at the beginning of the test, and the agent would receive an RGB-D image at every subsequent step. For the available actions, we set \texttt{move forward} to $0.25$ m and \texttt{rotate} to $30$ degrees. The task was defined as follows: an embodied agent with an egocentric-view camera and microphone hears an unknown object fall somewhere in the room it is in (a study room or kitchen) as shown in Figure~\ref{simulation}; the agent is then required to integrate audio-visual information to find which object has fallen and where it is, as efficiently as possible. Audio is recorded at $44.1$ kHz in a two-channel configuration. We generate the STFT representation using a window and FFT size of $512$, a hop length of $128$, and a Hann window. The PSD representation is generated using Welch’s method with a Hann window of size $256$, an overlap of $128$, and FFT size of $256$.

We evaluate agents using three metrics: Success Rate, Success weighted by Path Length (SPL) \cite{anderson2018evaluation}, and Success weighted by Number of Actions (SNA) \cite{chen2020learning}. The Success Rate is calculated as the ratio of successful navigation trials to the total number of trials. A trial is considered successful if the agent explicitly executes action \texttt{found} when the distance between the agent and the object is less than 2 meters, the target physical object is visible in the agent's view, and the number of actions executed so far is less than the maximum number of allowed steps (set to 200 in all tests). SPL is a metric that jointly considers the success rate and the path length to reach the goal from the starting point. SNA takes into account the number of actions and the success rate, penalizing collisions, rotations, and height adjustments taken to find the targets.



\input{tabletext/results_main}

\input{figtext/uncertainty_map}

\noindent\textbf{Result analysis.}
We evaluate the effectiveness of our proposed method against strong baselines as proposed in \cite{gan2022finding}. In Table~\ref{resultmain}, we find that our disentangled model based method can significantly outperform the previous modular planning baseline by $14\%$ absolute in success rate. We further observe a significant decrease in the average length of the path and the number of actions taken by the agents. In addition, we test the method that firstly navigates to the location predicted by the encoder, and then utilizes the loss map for further exploration if the first attempt fails. In this case, we observe a comparable SR, but lower SPL and SNA metrics, which highlights the effectiveness of the loss map in exploration.
We visualize the loss map and trajectories taken by the agent in Figure~\ref{lossmap}. We observe in Figure~\ref{lossmap} (a)$\sim$(f) that the modular planner often fails to find the target and attempts to find the object via random search, while our method can plan a direct route to the object. In Figure~\ref{lossmap} (g)$\sim$(h), both methods find the target, but our method takes a shorter path. These results illustrate the superiority of our proposed approach over the baseline modular planner. 

\vspace{1mm}
\noindent\textbf{Ablation studies.}
The modular nature of our proposed method facilitates ablation studies that yield insight into the contribution of each individual component. We report results for ablations in Table~\ref{resultmain}. Beginning with the modular planning baseline, we find that augmenting the planner with a loss-map-guided object priority ranker yields a  2$\%$ increase in SR, a 3$\%$ increase in SPL, and 4$\%$ increase in SNA. This shows that the introduction of the uncertainty map can effectively improve the efficiency of agents searching for potential objects, reducing both the length of the path and the number of actions taken. Additionally, we replaced the sound location and sound type predictors in modular planning with our predictor jointly trained with a generator. The improvement in the object type prediction accuracy was found to contribute more to the overall SR than the improvement in the position accuracy. This result corroborates the conclusion in \cite{gan2022finding} that accurately predicting object types from audio alone is a major challenge.
\input{tabletext/cross_accuracy}
\input{tabletext/generalization}

% Our ablation experiments have yielded valuable insights into the factors that contribute to the improvement. We added a loss surface to the modular planning method to set the priority of approaching potential objects, resulting in a 2$\%$ increase in SR, a 3$\%$ increase in SPL and 4$\%$ increase in SNA. This shows that the introduction of the uncertainty surface can effectively improve the efficiency of agents searching for potential objects, reducing both the length of the path and the number of actions taken. Additionally, we replaced the sound location and sound type predictors in modular planning with our own network, respectively. The improvement in the object type prediction accuracy was found to contribute more to the overall SR than the improvement in the position accuracy. This result corroborates \cite{gan2022finding}'s conclusion that accurately predicting object types from audio alone is a major challenge.


\vspace{1mm}
\noindent\textbf{Cross-Scene Generalization.}
% The results of Decision TransFormer \cite{chen2021decision}, PPO (Oracle found) \cite{schulman2017proximal} and Object-Goal \cite{chaplot2020object} are taken from \cite{gan2022finding}.
To explicitly assess the generalization ability of our proposed method, we train and test on entirely different classes of rooms. In the first split, models are trained in the kitchens and tested in the study rooms. For the second split, models are trained in the study rooms and tested in the kitchens. The object property prediction results are reported in Table~\ref{predict2}. In both splits, the accuracy of positioning and predicting the type of object slightly decreased compared to that of the full-trained model. The planning results are reported in Table~\ref{cross_scene}, where all models experience a degree of cross-scene performance drop. The success rate of the modular planning approach decreases by $7\%$ in SR on the first split, while our method only decreases by $4\%$. Our proposed method still performs the best in both splits. This highlights that our method can not only generalize across room instances of the same type, but can also effectively generalize across rooms of a different type.



% \begin{figure*}
% 		\centering
% 		\includegraphics[scale=0.49]{fig/seg.pdf}
% 		\caption{
% This figure depicts examples of semantic segmentation errors. Above four figures are first-person view images from the agent and the below fours images are their corresponding semantic segmentation results. The incorrect recognition can be attributed to the object's small size, or shape and color being poorly distinguished from the background.  }
% 		\label{seg}
% 	\end{figure*}



%here
% \input{figtext/failure_1}
% \input{figtext/failure_2}

% \vspace{2mm}
% \noindent\textbf{Failure Case Analysis.}
% Despite significant performance improvements upon baseline methods, our methods still may sometimes fail to find the fallen object. Upon analyzing some cases, we discover that inaccurate semantic segmentation is one major problem. In such scenes, even if the target position and type are accurately predicted by our audio network, the agent would not be able to find the object. As illustrated in Figure~\ref{seg}, some segmentation failures are due to the object being too small, or it being too close to the background color. Additionally, distractor objects may cause the agent to use the \texttt{found} command on the wrong object. 
% We show two trajectories where our method cannot find the object or uses a long path. 
% Figure~\ref{failure} (a) shows a case where multiple distractors of the same kind as the fallen object are in the agent's view, and thus both the baseline and our method fail to navigate to the target location. As seen in Figure~\ref{failure} (b), the introduction of a loss map does not necessarily ensure that the agent takes the shortest path. Our method succeeds in finding the target, but it takes a longer path than the baseline. 





% Finally, we find another potential cause of unsuccessful navigation: the robot got stuck in a tight corner and couldn't get out within the limited moving directions. Although such cases do not happen frequently in our experiments, this discovery enlighten us to pay attention to the importance of path planning and safe exploration. 




% Similar to other embodied AI challenges, we also hope to build autonomous navigation agents that generalize to unseen scenarios. To explicitly test agents’ generalization abilities, we define two splits of the training set and test set for cross-scene evaluation. In the first split, the models are trained in the study rooms but tested in the kitchens. In the second split, we train models in the kitchens but test them in the study rooms. The results are reported in Table2. All models have some degree of cross-scene performance drop. For example, the success rate of the modular planning approach decreased by 6$\%$. We analyzed some failure cases and found that most of them come from the visual percep-
% tion module. For example, the Mask-RCNN network some-
% times fails to detect the fallen objects lying on a different
% color carpet, which requires agents to take additional time
% steps to find it.




% \subsection{Evaluation on Distractor Senarios}

==> sections/05_Conclusion.tex <==
\vspace{-0.2em}
\section{Conclusion}
This paper presents an egocentric disentangled acoustic field framework that can generalize and reason across scenes. Joint inference of sound properties is implemented by using an explicit decomposition in the latent space. Furthermore, our approach is capable of generating multimodal uncertainty maps. Experiments on the TDW simulation platform demonstrate our disentangled acoustic field can improve the success rate for the localization of fallen objects. Consequently, our proposed method is a promising solution for sound localization and understanding in complex scenes.

% \paragraph{Future Work}
% We are interested in agents that possess audio-visual sound source separation capabilities. To this end, we intend to extend the Fallen Object Dataset and incorporate synthetic distractor sounds into the scene. These sounds can be generated from various object interactions in the environment, necessitating that the agent can recognize which combination of objects will produce the specified audio-goal. For example, if a TV remote control device were to fall in a living room, the agent would have to identify and separate the sound of the falling object from the background television sound before navigating.


